ltzGLUE: Luxembourgish General Language Understanding Evaluation

This paper presents ltzGLUE, the first Natural Language Understanding (NLU) benchmark for Luxembourgish (LTZ) based on the popular GLUE benchmark for English. Although NLU tasks are available for many European languages nowadays, LTZ is one of the official national languages that is often overlooked. We construct new tasks and reuse existing ones to introduce the first official NLU benchmark and accompanying evaluation of encoder models for the language. Our tasks include common natural language processing tasks in binary and multi-class classification settings, including named entity recognition, topic classification, and intent classification. We evaluate various pre-trained language models for LTZ to present an overview of the current capabilities of these models on the LTZ language.

==> tables/hc_results.tex <==
\begin{table}[t]
\centering
\begin{tabular}{@{}ll}
\toprule
\textbf{Model} & \textbf{Test \Fone} \\
\midrule
\luxembert & \cellcolor[HTML]{E5F5ED}\fonesd{66.37}{0.00} \\
\mbert & \cellcolor[HTML]{90D2B2}\fonesd{77.91}{10.26} \\
\modelname-base & \cellcolor[HTML]{FFFFFF}\fonesd{62.81}{4.98} \\
\modelname-mini & \cellcolor[HTML]{B7E2CD}\fonesd{72.69}{1.33} \\
\mmbert & \cellcolor[HTML]{57BB8A}\fonesd{85.59}{1.61} \\
\roberta & \cellcolor[HTML]{BBE4D0}\fonesd{72.09}{9.90} \\ 
\bottomrule
\end{tabular}%
\caption{\textbf{Test \Fone scores for the headline acceptability task}. Results are averaged over three runs, with standard deviations as subscripts.}
\label{tab:hc_results}
\end{table}

==> tables/lab_results.tex <==
\begin{table}[]
\centering
\begin{tabular}{@{}ll}
\toprule
\textbf{Model} & \textbf{Test \Fone} \\
\midrule
\luxembert & \cellcolor[HTML]{5EBE8F}\fonesd{89.17}{0.18} \\
\mbert & \cellcolor[HTML]{A2DABE}\fonesd{81.26}{0.56} \\
\modelname-base & \cellcolor[HTML]{91D3B3}\fonesd{83.17}{8.38} \\
\modelname-mini & \cellcolor[HTML]{5DBE8E}\fonesd{89.31}{2.89} \\
\mmbert & \cellcolor[HTML]{57BB8A}\fonesd{89.97}{0.09} \\
\roberta & \cellcolor[HTML]{FFFFFF}\fonesd{70.25}{4.55} \\
\bottomrule
\end{tabular}
\caption{\textbf{Test \Fone scores for the binary linguistic acceptability task}. Results are averaged over three runs, with standard deviations as subscripts.}
\label{tab:lab_results}
\end{table}

==> tables/lam_results.tex <==
\begin{table}[]
\centering
\begin{tabular}{@{}ll}
\toprule
\textbf{Model} & \textbf{Test \Fone} \\
\midrule
\luxembert & \cellcolor[HTML]{6EC59A}\fonesd{87.96}{0.71} \\
\mbert & \cellcolor[HTML]{AEDFC7}\fonesd{81.20}{1.02} \\
\modelname-base & \cellcolor[HTML]{C6E8D8}\fonesd{78.63}{11.55} \\
\modelname-mini & \cellcolor[HTML]{7BCAA3}\fonesd{86.62}{4.64} \\
\mmbert & \cellcolor[HTML]{57BB8A}\fonesd{90.35}{0.72} \\
\roberta & \cellcolor[HTML]{FFFFFF}\fonesd{72.59}{2.69} \\ \bottomrule
\end{tabular}
\caption{\textbf{Test \Fone scores for the multiclass linguistic acceptability task}. Results are averaged over three runs, with standard deviations as subscripts.}
\label{tab:lam_results}
\end{table}

==> tables/ner_results.tex <==
\begin{table}[]
\centering
\begin{tabular}{@{}ll}
\toprule
\textbf{Model} & \textbf{Test \Fone} \\
\midrule
\luxembert & \cellcolor[HTML]{6BC398}\fonesd{90.57}{0.09}\\
\mbert & \cellcolor[HTML]{5FBE90}\fonesd{90.83}{0.28}\\
\modelname-base & \cellcolor[HTML]{AEDFC7}\fonesd{89.17}{0.70}\\
\modelname-mini & \cellcolor[HTML]{FFFFFF}\fonesd{87.47}{0.37}\\
\mmbert & \cellcolor[HTML]{57BB8A}\fonesd{90.98}{0.23}\\
\roberta & \cellcolor[HTML]{90D2B2}\fonesd{89.80}{0.50}\\
\bottomrule
\end{tabular}
\caption{\textbf{Test \Fone scores for the named entity recognition task}. Results are averaged over three runs, with standard deviations as subscripts.}
\label{tab:ner_results}
\end{table}

==> tables/rte_results.tex <==
\begin{table}[]
\centering
\begin{tabular}{@{}ll}
\toprule
\textbf{Model} & \textbf{Test \Fone} \\
\midrule
\luxembert & \cellcolor[HTML]{94D4B5}\fonesd{70.96}{0.26}\\
\mbert & \cellcolor[HTML]{72C69D}\fonesd{73.48}{1.84}\\
\modelname-base & \cellcolor[HTML]{BEE5D2}\fonesd{67.88}{3.20}\\
\modelname-mini & \cellcolor[HTML]{FFFFFF}\fonesd{63.10}{3.64}\\
\mmbert & \cellcolor[HTML]{57BB8A}\fonesd{75.44}{2.41}\\
\roberta & \cellcolor[HTML]{96D5B6}\fonesd{70.82}{0.42}\\
\bottomrule
\end{tabular}
\caption{\textbf{Test \Fone scores for the textual entailment task}. Results are averaged over three runs, with standard deviations as subscripts.}
\label{tab:rte_results}
\end{table}

==> tables/sa_results.tex <==
% CAREFUL THESE ARE OLD, full_results has groundtruth
\begin{table}[]
\centering
\begin{tabular}{@{}ll}
\toprule
\textbf{Model} & \textbf{Test \Fone} \\
\midrule
\luxembert & \cellcolor[HTML]{57BB8A}\fonesd{55.12}{1.67}\\
\mbert & \cellcolor[HTML]{C5E8D7}\fonesd{42.16}{0.38}\\
\modelname-base & \cellcolor[HTML]{DCF1E7}\fonesd{39.38}{6.04}\\
\modelname-mini & \cellcolor[HTML]{AADDC4}\fonesd{45.35}{ 5.71}\\
\mmbert & \cellcolor[HTML]{6BC398}\fonesd{52.81}{3.01}\\
\roberta & \cellcolor[HTML]{FFFFFF}\fonesd{35.24}{7.73}\\
\bottomrule
\end{tabular}
\caption{\textbf{Test \Fone scores for the semantic analysis task}. Results are averaged over three runs, with standard deviations as subscripts.}
\label{tab:sa_results}
\end{table}

==> tables/sid_results.tex <==
\begin{table}[]
\centering
\begin{tabular}{@{}ll}
\toprule
\textbf{Model} & \textbf{Test \Fone} \\
\midrule
\luxembert & \cellcolor[HTML]{57BB8A}\fonesd{91.71}{0.11 }\\
\mbert & \cellcolor[HTML]{FFFFFF}\fonesd{60.65}{4.71 }\\
\modelname-base & \cellcolor[HTML]{BBE4D0}\fonesd{73.32}{11.66 }\\
\modelname-mini & \cellcolor[HTML]{96D5B6}\fonesd{80.13}{3.00 }\\
\mmbert & \cellcolor[HTML]{A0D9BD}\fonesd{78.26}{7.22 }\\
\roberta & \cellcolor[HTML]{F4FBF8}\fonesd{62.75}{8.76 }\\
\bottomrule
\end{tabular}
\caption{\textbf{Test \Fone scores for the intent detection task}. Results are averaged over three runs, with standard deviations as subscripts.}
\label{tab:sid_results}
\end{table}

==> tables/tc_results.tex <==
\begin{table}[]
\centering
\begin{tabular}{@{}ll}
\toprule
\textbf{Model} & \textbf{Test \Fone} \\
\midrule
\luxembert & \cellcolor[HTML]{72C69D}\fonesd{98.68}{0.17}\\
\mbert & \cellcolor[HTML]{C8E9D9}\fonesd{97.80}{0.67}\\
\modelname-base & \cellcolor[HTML]{57BB8A}\fonesd{98.95}{0.36}\\
\modelname-mini & \cellcolor[HTML]{84CDA9}\fonesd{98.50}{0.23}\\
\mmbert & \cellcolor[HTML]{5BBD8D}\fonesd{98.92}{0.28}\\
\roberta & \cellcolor[HTML]{FFFFFF}\fonesd{97.24}{0.50}\\
\bottomrule
\end{tabular}
\caption{\textbf{Test \Fone scores for the topic classification task}. Results are averaged over three runs, with standard deviations as subscripts.}
\label{tab:tc_results}
\end{table}
